Variable Independence in Linear Real Arithmetic

Variable independence and decomposability are algorithmic techniques for simplifying logical formulas by tearing apart connections between free variables. These techniques were originally proposed to speed up query evaluation in constraint databases, in particular by representing the query as a Boolean combination of formulas with no interconnected variables. They also have many other applications in SMT, string analysis, databases, automata theory and other areas. However, the precise complexity of variable independence and decomposability has been left open especially for the quantifier-free theory of linear real arithmetic (LRA), which is central in database applications. We introduce a novel characterization of formulas admitting decompositions and use it to show that it is coNP-complete to decide variable decomposability over LRA. As a corollary, we obtain that deciding variable independence is in $ \Sigma_2^p $. These results substantially improve the best known double-exponential time algorithms for variable decomposability and independence. In many practical applications, it is crucial to be able to efficiently eliminate connections between variables whenever possible. We design and implement an algorithm for this problem, which is optimal in theory, exponentially faster compared to the current state-of-the-art algorithm and efficient on various microbenchmarks. In particular, our algorithm is the first one to overcome a fundamental barrier between non-discrete and discrete first-order theories. Formulas arising in practice often have few or even no free variables that are perfectly independent. In this case, our algorithm can compute a best-possible approximation of a decomposition, which can be used to optimize database queries by exploiting partial variable independence, which is present in almost every logical formula or database query constraint.

==> abstract.tex <==
Intuitively, two variables in some logical formula are said to be independent, if there exists a way of equivalently rewriting the formula so that no predicate connects both variables. More generally, people study the notion of variable decomposability, which asks whether the given formula can be rewritten as a Boolean combination of predicates each having its free variables within some block of a partition. Decision procedures for these problems have applications in SMT and string analysis \cite{veanes:2017}, databases \cite{libkin:2000, libkin:2003}, automata theory \cite{barcelo:2019} and other areas. However, not much is known about the computational complexity of these problems for many first-order theories -- this is an open problem raised in \cite{veanes:2017}. In this paper we study the variable decomposition and independence problems over the quantifier-free fragment of Linear Real Arithmetic (LRA). We introduce a novel characterization of formulas admitting decompositions, which we use to show that deciding decomposability is $ \coNP $-complete. As a corollary, we obtain that the variable decomposition and independence problems are $ \coNP $-complete and in $ \NP^\NP $, respectively. This substantially improves the best known double-exponential time algorithm for both problems. We apply the same characterization to show a practical way of deciding variable decomposability which, unlike many other approaches, yields not just a yes/no answer to a decomposability question, but is capable of actually producing the variable decomposition if one exists. This further enhances the applicability of our algorithm, which, as experiments have shown, is moreover also efficient in practice.


==> commands_paper.tex <==
% Use bullets in itemize
\let\labelitemi\labelitemii

% Prevent italic capital Greek letters in math mode
% we can still use e.g. \mathnormal{\Sigma} to obtain the italic version of a Greek letter
\DeclareMathSymbol{\Gamma}{\mathalpha}{operators}{0}
\DeclareMathSymbol{\Delta}{\mathalpha}{operators}{1}
\DeclareMathSymbol{\Theta}{\mathalpha}{operators}{2}
\DeclareMathSymbol{\Lambda}{\mathalpha}{operators}{3}
\DeclareMathSymbol{\Xi}{\mathalpha}{operators}{4}
\DeclareMathSymbol{\Pi}{\mathalpha}{operators}{5}
\DeclareMathSymbol{\Sigma}{\mathalpha}{operators}{6}
\DeclareMathSymbol{\Upsilon}{\mathalpha}{operators}{7}
\DeclareMathSymbol{\Phi}{\mathalpha}{operators}{8}
\DeclareMathSymbol{\Psi}{\mathalpha}{operators}{9}
\DeclareMathSymbol{\Omega}{\mathalpha}{operators}{10}

\spnewtheorem{zbclaim}[theorem]{Claim}{\bfseries}{}
\spnewtheorem{zbdefinition}[definition]{Definition}{\bfseries}{}
\spnewtheorem{zbexample}[theorem]{Example}{\bfseries}{}
\spnewtheorem{zbproblem}[theorem]{Problem}{\bfseries}{}

\def\zbdocname/{paper}
\def\zbsectionname/{section}

\newcommand{\zbthesismode}{0}
\newcommand{\zbtikzbiggerscaling}{1.2}
\newcommand{\zbtikznormalscaling}{1}
\newcommand{\zbtikzaggressivescaling}{1}
\newcommand{\zbrefsec}[1]{Section~\ref{#1}}

==> deprecated/normal_form.tex <==
In this section, we prove some facts about the normal form we introduced, with the primary goal of establishing Lemma~\ref{lemma:every_disj_either_true_or_false}.

\begin{lemma}
	\label{lemma:model_indistinguishability}
	Let $ \psi_1 $, $ \psi_2 $ be satisfiable formulas such that $ \psi_1, \psi_2 \models \Theta $ for some $ \Theta \in \DisjTrue $. Then $ \psi_1 \models \varphi $ is equivalent to $ \psi_2 \models \varphi $.
\end{lemma}
\begin{proof}
	It suffices to show the ``$ \Rightarrow $'' direction, because the the proof of the converse implication is symmetric. Suppose $ \psi_1 \models \varphi $. Since $ \psi_1 $ is satisfiable and \[
	\psi_1 \models \varphi \equiv \bigvee_{\Gamma \in \DisjPhi} \Gamma
	\] there exists $ v \models \psi_1 \wedge \Gamma $ for some $ \Gamma \in \DisjPhi $. At the same time, $ v \models \psi_1 \models \Theta $. It follows that $ \Gamma = \Theta $, because $ \Gamma $ and $ \Theta $ agree on $ v \models \Gamma \cup \Theta $, but no two distinct disjuncts in $ \DisjTrue $ can agree on any model. Hence, $ \Theta = \Gamma \models \varphi $, from which we immediately get $ \psi_2 \models \Theta \models \varphi $.
\end{proof}

\begin{corollary}
	\label{cor:model_indistinguishability}
	Let $ \psi $ be a satisfiable formula such that $ \psi \models \Theta $ for some $ \Theta \in \DisjTrue $. Then $ \psi \wedge \varphi $ is satisfiable if and only if $ \psi \models \varphi $.
\end{corollary}
\begin{proof}
	The ``$ \Leftarrow $'' direction is clear. The converse holds, because by Lemma~\ref{lemma:model_indistinguishability} applied to satisfiable formulae $ \psi_1 := \psi \wedge \varphi $ and $ \psi_2 := \psi $, the trivial entailment $ \psi \wedge \varphi \models \varphi $ is equivalent to $ \psi \models \varphi $.
\end{proof}

Having done the above preparatory work, we now prove Lemma~\ref{lemma:every_disj_either_true_or_false}. Clearly, either $ \Theta \wedge \varphi $ or $ \Theta \wedge \neg\varphi $ must be satisfiable. In the former case, by Corollary \ref{cor:model_indistinguishability} we obtain that $ \Theta \models \varphi $, whereas in the latter case Corollary \ref{cor:model_indistinguishability} yields $ \Theta \models \neg\varphi $. This completes the proof.

==> deprecated/pi_complex.tex <==
\subsection{Nelson-Oppen Convexity}

For one of the proofs, we will need the following result, which is essentially a refined version of the well-known notion of convexity introduced by Nelson and Oppen in the context of constructing decision procedures for a combination of first-order theories \cite{nelson_oppen:1979, oppen:1980, bruttomesso:2009:nelson_oppen}. The same notion is discussed in the context of linear real arithmetic also, for example, in \cite[pp. 230, 231]{kroening:2016}.

\begin{lemma}[Nelson-Oppen Convexity \cite{nelson_oppen:1979, oppen:1980}]
	\label{lemma:no_convexity}
	Let $ \Gamma $ be a predicate set and $ p_1, \dots, p_n $ be equality predicates such that \[
	\Gamma \models \bigvee_{i=1}^n p_i
	\] Then, there exists $ i \in \{1, \dots, n\} $ such that $ \Gamma \models p_i $.
\end{lemma}
\begin{proof}
	See \cite[pp. 299, 300]{oppen:1980}.
\end{proof}

\subsection{Disjunction over $ \Pi $-simple predicate sets is $ \Pi $-simple}

Building on top of Lemma~\ref{lemma:no_convexity}, we now prove that, intuitively, a finite union of sets defined by $ \Pi $-simple predicate sets must also be $ \Pi $-simple.

\begin{lemma}
	\label{lemma:union_of_pi_simple_regions_is_pi_simple}
	Let $ \Lambda, \Lambda_1, \dots, \Lambda_k $ be predicate sets such that $ \Lambda \equiv \bigvee_{i = 1}^k \Lambda_i $. Then $ \Lambda $ is $ \Pi $-simple if and only if $ \Lambda_i $ is $ \Pi $-simple for all $ 1 \le i \le k $.
\end{lemma}
\begin{proof}
	The ``$ \Rightarrow $'' direction is easy: for every $ i $ we have that $ \Lambda_i \models \Lambda $, so $ \Fixes(\Lambda) \subseteq \Fixes(\Lambda_i) $. Hence, $ \Lambda $ being $ \Pi $-simple implies that $ \Lambda_i $ is $ \Pi $-simple.
	
	For the ``$ \Leftarrow $'' direction, we assume that every $ \Lambda_i $ is $ \Pi $-simple and, w.l.o.g., that $ \Lambda $ is satisfiable.
	\begin{zbclaim}
		\label{claim:lambda_fixes_x1_or_x2}
		For every distinct $ X_1, X_2 \in \Pi $ and $ i \in \{1, \dots, k\} $, $ \Lambda_i $ fixes either $ X_1 $ or $ X_2 $.
	\end{zbclaim}
	\begin{proof}
		Follows immediately from the fact that $ \Lambda_i $ is $ \Pi $-simple for all $ 1 \le i \le k $.
	\end{proof}
	
	By Claim~\ref{claim:lambda_fixes_x1_or_x2}, for every distinct $ X_1, X_2 \in \Pi $ there exists a function $ \sigma : \{1, \dots, k\} \rightarrow \{1, 2\} $ such that for all $ i \in \{1, \dots, k\} $, $ \Lambda_i $ fixes $ X_{\sigma(i)} $. We now let $ X_1, X_2 \in \Pi, X_1 \neq X_2 $ be arbitrary but fixed. Let $ \mu : X_1 \cup X_2 \rightarrow \Q $ be a function mapping $ x \in X_i $, $ i \in \{1, 2\} $ to the value $ \Lambda_i $ fixes for the variable $ x $. Note that $ \mu $ is well-defined, because $ X_1 \cap X_2 = \varnothing $. Since $ \Lambda \models \bigvee_{i = 1}^k \Lambda_i $, \begin{align}
		\label{eqn:lambda_entails_variable_fixing}
		\Lambda \models \bigvee_{i = 1}^k \bigwedge_{x \in X_{\sigma(i)}} x = \mu(x)
	\end{align} because every $ \Lambda_i $ entails $ \bigwedge_{x \in X_{\sigma(i)}} x = \mu(x) $.
	
	Fix some total ordering $ \prec $ on the variables $ x_1, \dots, x_n $ of $ \varphi $. We can assume without loss of generality that for every $ i \in \{1, 2\} $, $ X_i = \{x_{f_i(1)}, \dots, x_{f_i(|X_i|)}\} $, where $ f_i : X_i \rightarrow \{1, \dots, n\} $ is a function mapping indices $ 1, \dots, |X_i| $ of elements of $ X_i $ to the corresponding variable indices, such that for every $ a, b \in \{1, \dots, |X_i|\} $, $ x_{f_i(a)} \prec x_{f_i(b)} $ if $ a < b $. In other words, this means that for every $ i \in \{1, 2\} $, $ x_{f_i(1)} \prec \dots \prec x_{f_i(|X_i|)} $. Let $ T := X_1 \times X_2 $. For every $ u := (u_1, u_2) \in T $, $ w := (w_1, w_2) \in T $ and $ i \in \{1, 2\} $, we write $ u \prec_i w $ if $ w_i = \min\{w \in X_i \mid u_i \prec w\} $ and $ u_j = w_j $ for $ j \neq i $.
	
	We now construct a finite sequence $ u_1 \prec_{j_1} u_2 \prec_{j_2} u_3 \prec_{j_3} \dots \prec_{j_{l-1}} u_l $ in $ T $ with the following property:
	
	\begin{zbclaim}
		\label{claim:prec_sequence_property}
		For every $ j $, if $ u_j = (y_1, y_2) \prec_i u_{j+1} $, then $ \Lambda $ fixes $ y_i $.
	\end{zbclaim}
	
	We construct the sequence inductively. Set $ u_1 := (x_{f_1(1)}, x_{f_2(1)}) $ to be the first element. Let $ u_j = (y_1, y_2) $ be the last element of the sequence so far. In the following, we either stop constructing the sequence at $ u_l = u_j $, or show how to construct the next element $ u_{j+1} $ such that the sequence satisfies Claim~\ref{claim:prec_sequence_property}. Weakening the conjunction in (\ref{eqn:lambda_entails_variable_fixing}) yields \begin{align}
		\label{eqn:lambda_entails_variable_fixing_weak}
		\Lambda \models \bigvee_{i = 1}^k y_{\sigma(i)} = \mu(y_{\sigma(i)})
	\end{align} because for every $ i \in \{1, \dots, k\} $, $ y_{\sigma(i)} \in X_{\sigma(i)} $. By Lemma~\ref{lemma:no_convexity} applied to (\ref{eqn:lambda_entails_variable_fixing_weak}), there exists an $ i \in \{1, \dots, k\} $ such that $ \Lambda \models y_{\sigma(i)} = \mu(y_{\sigma(i)}) $. Hence, $ \Lambda $ fixes $ y_i $.
	
	\begin{zbclaim}
		\label{claim:succ_empty_completes_proof}
		If at this point $ y_i = \max_\prec{X_i} $, then this completes the proof of Lemma~\ref{lemma:union_of_pi_simple_regions_is_pi_simple}.
	\end{zbclaim}
	
	By Claim~\ref{claim:succ_empty_completes_proof}, we can without loss of generality assume that $ \{z \in X_i \mid y_i \prec z\} \neq \varnothing $. It follows that \[
	u_{j+1} := \begin{cases}
		(z_1, y_2), & \text{if } i = 1 \\
		(y_1, z_2), & \text{if } i = 2
	\end{cases}
	\] where $ z_i := \min\{z \in V_i \mid y_i \prec z\} $, is well-defined. We conclude that the above construction either completes the proof of Lemma~\ref{lemma:union_of_pi_simple_regions_is_pi_simple} by Claim~\ref{claim:succ_empty_completes_proof}, or ensures that the constructed sequence satisfies Claim~\ref{claim:prec_sequence_property}.
	
	Now observe that the above construction of the sequence ensures, that if $ u_j = (y_1, y_2) $ is an element of the sequence (for some $ j $), then $ x_{f_1(1)} \prec y_1 $ and $ x_{f_2(1)} \prec y_2 $. In words, this simply means that as we keep constructing new elements of the sequence, its components can only increase (with respect to the $ \prec $ order) or stay unchanged. Since the domain $ T $ of the sequence is finite, its elements have only two components, one of which is guaranteed to increase in every step, it follows that there exists an element of the sequence with a maximal component. Hence, the condition of Claim~\ref{claim:succ_empty_completes_proof} is guaranteed to become true after finitely many steps. Thus, to complete the proof of Lemma~\ref{lemma:union_of_pi_simple_regions_is_pi_simple} it suffices to show Claim~\ref{claim:succ_empty_completes_proof}, which we do in the remainder of the proof.
	
	Suppose that at some point in the sequence, $ y_i = \max_\prec{X_i} $ holds. Note that in every step of the sequence, if some component gets increased, then it gets increased to the smallest value exceeding it, with respect to the $ \prec $ order. Hence, $ y_i = \max_\prec{X_i} $ taken together with Claim~\ref{claim:prec_sequence_property} implies that $ \Lambda $ fixes $ X_i $.
	
	Now suppose, for the sake of contradiction, that $ \Lambda $ were $ \Pi $-complex. This means that there exist at least two distinct $ X_1, X_2 \in \Pi $ such that $ \Lambda $ fixes neither $ X_1 $ nor $ X_2 $. By Claim~\ref{claim:lambda_fixes_x1_or_x2}, $ \Lambda_i $ fixes either $ X_1 $ or $ X_2 $, for all $ i \in \{1, \dots, k\} $. From this we have derived above that $ \Lambda $ fixes $ X_i $ for some $ i \in \{1, 2\} $. This is a contradiction.
\end{proof}

\subsection{Strict inequalities cannot make a predicate set $ \Pi $-simple}

\begin{lemma}
	\label{lemma:adding_neq_predicates_cannot_make_pi_complex_set_pi_simple}
	Let $ \Gamma $ be a $ \Pi $-complex predicate set and let $ p $ be a predicate. Then $ \Gamma \cup \{p^<\} $ is $ \Pi $-complex if $ \Gamma \cup \{p^<\} $ is satisfiable and $ \Gamma \cup \{p^>\} $ is $ \Pi $-complex if $ \Gamma \cup \{p^>\} $ is satisfiable.
\end{lemma}
\begin{proof}
	Suppose $ \Gamma \cup \{p\} $ were satisfiable, and, for a sake of contradiction, that $ \Gamma \cup \{p\} $ were $ \Pi $-simple. Since \[
	(\Gamma \cup \{p\})^= = \Gamma^= \subsetneq (\Gamma \cup \{p[P_{\neq}/P_=]\})^=
	\] by Corollary \ref{cor:fixing_eq_inclusion_implies_inclusion}, $ \Fixes(\Gamma \cup \{p\}) \subseteq \Fixes(\Gamma \cup \{p[P_{\neq}/P_=]\}) $. Hence, $ \Gamma \cup \{p[P_{\neq}/P_=]\} $ is $ \Pi $-simple. Now observe that since $ p \equiv \neg p[P_{\neq}/P_=] $, $ \Gamma $ can be written as the following disjunction of $ \Pi $-simple predicate sets: \[
	\Gamma \equiv (\Gamma \cup \{p\}) \vee (\Gamma \cup \{p[P_{\neq}/P_=]\})
	\] Hence, by Lemma~\ref{lemma:union_of_pi_simple_regions_is_pi_simple}, $ \Gamma $ is $ \Pi $-simple, which is a contradiction.
\end{proof}

==> deprecated/util.tex <==
\begin{corollary}
	\label{cor:lindep_eq_equality_implies_equality}
	Let $ \Gamma_1, \Gamma_2 $ be satisfiable sets of predicates, $ V $ be a $ \Q $-vectorspace and $ h : \Q^n \rightarrow V $ be a $ \Q $-vectorspace homomorphism. Suppose furthermore that $ \Gamma_1^= = \Gamma_2^= $. Then \[
	\LinDep_{h, v}(\Gamma_1) = \LinDep_{h, v}(\Gamma_2)
	\] holds for all $ v \models \Gamma_1^= $.
\end{corollary}
\begin{proof}
	Corollary \ref{cor:lindep_eq_inclusion_implies_inclusion} applied to $ (\Gamma_1, \Gamma_2) $ and to $ (\Gamma_2, \Gamma_1) $.
\end{proof}

==> deprecated/util_lemmas.tex <==
\subsection{Fixed variables and linear dependencies}

\textcolor{red}{TODO: polish}

\begin{corollary}
	\label{cor:lindep_eq_inclusion_implies_inclusion}
	Let $ \Gamma_1, \Gamma_2 $ be satisfiable sets of predicates, $ V $ be a $ \Q $-vectorspace and $ h : \Q^n \rightarrow V $ be a $ \Q $-vectorspace homomorphism. Then for all $ v \models \Gamma_1^= $ it holds that \[
	\LinDep_{h, v}(\Gamma_1) \subseteq \LinDep_{h, v}(\Gamma_2)
	\] if $ \Gamma_1^= \subseteq \Gamma_2^= $.
\end{corollary}
\begin{proof}
	Suppose $ \Gamma_1^= \subseteq \Gamma_2^= $. This implies $ \Gamma_2^= \models \Gamma_1^= $ and hence \[
	h(\ModelsOf(\Gamma_2^=) - v) \subseteq h(\ModelsOf(\Gamma_1^=) - v)
	\] It follows that \begin{align}
		\label{eqn:gamma1eq_lindep_subsetof_gamma2eq_lindep}
		\LinDep_{h, v}(\Gamma_1^=) \subseteq \LinDep_{h, v}(\Gamma_2^=)
	\end{align} Similarly, from $ \Gamma_2 \models \Gamma_2^= $ we obtain \begin{align}
		\label{eqn:gamma2eq_lindep_subsetof_gamma2_lindep}
		\LinDep_{h, v}(\Gamma_2^=) \subseteq \LinDep_{h, v}(\Gamma_2)
	\end{align} Combining the above inclusions with Theorem~\ref{thm:only_equality_predicates_can_establish_lindep_strong} yields \[
	\LinDep_{h, v}(\Gamma_1) \overset{\ref{thm:only_equality_predicates_can_establish_lindep_strong}}{=} \LinDep_{h, v}(\Gamma_1^=) \overset{(\ref{eqn:gamma1eq_lindep_subsetof_gamma2eq_lindep})}{\subseteq} \LinDep_{h, v}(\Gamma_2^=) \overset{(\ref{eqn:gamma2eq_lindep_subsetof_gamma2_lindep})}{\subseteq} \LinDep_{h, v}(\Gamma_2)
	\] as desired.
\end{proof}

\begin{corollary}
	\label{cor:fixing_eq_inclusion_implies_inclusion}
	Let $ \Gamma_1, \Gamma_2 $ be satisfiable sets of predicates. Then $ \Fixes(\Gamma_1) \subseteq \Fixes(\Gamma_2) $ if $ \Gamma_1^= \subseteq \Gamma_2^= $.
\end{corollary}
\begin{proof}
	Suppose $ \Gamma_1^= \subseteq \Gamma_2^= $ and take some $ x_i \in \Fixes(\Gamma_1) $. In terms of linear dependencies, this means that $ \gen{e_i} \in \LinDep_{\id, v}(\Gamma_1) $ for all $ v \models \Gamma_1 $, where $ e_i $ is the $ i $-th canonical basis vector. By Theorem~\ref{thm:only_equality_predicates_can_establish_lindep_strong}, $ \gen{e_i} \in \LinDep_{\id, v}(\Gamma_1) $ for all $ v \models \Gamma_1^= $. By Corollary \ref{cor:lindep_eq_inclusion_implies_inclusion}, $ \gen{e_i} \in \LinDep_{\id, v}(\Gamma_2) $ holds for all $ v \models \Gamma_1^= $. Since \[
	\Gamma_2 \models \Gamma_2^= \models \Gamma_1^=
	\] it follows that $ \gen{e_i} \in \LinDep_{\id, v}(\Gamma_2) $ holds in particular for all $ v \models \Gamma_2 $. Hence, $ x_i \in \Fixes(\Gamma_2) $.
\end{proof}

==> packages_paper.tex <==
\hypersetup{
	pdftitle={Variable Independence in Linear Real Arithmetic},
	pdfauthor={Alexander Mayorov, Anthony W. Lin}
}

% Captions

\usepackage{caption}
\usepackage{subcaption}

% Bibliography

\usepackage[square,numbers]{natbib}

% \bibliographystyle{unsrtnat}

% use LNCS bibliography
\bibliographystyle{splncs04}

==> sections/intro_anthony.tex <==
\newcommand{\Partition}{\Pi}
\newcommand{\theory}{\mathcal{T}}
Consider a first-order formula $\varphi$ over some theory $\theory$.
The problem of
\emph{variable decomposability} (a.k.a. \emph{variable partitioning}) with
respect to the partition $\Partition := \{X_i\}_{i=1}^n$ of the free variables
in $\varphi$ (i.e. $X_i$'s are pairwise disjoint) is to decide if $\varphi$ can 
be written as a Boolean combination of formulas in $\theory$ of the form 
$\psi(X_i)$, i.e., that $\varphi$ can be decomposed into formulas that only
refer solely to one of the $X_i$'s. For example, the
following formula in Linear Real Arithmetic (LRA) 
\[
x + 3y + 9z \geq 0 \wedge y + 3z = 7
\]
admits variable independence with respect to the partition $\Pi =
(\{x\},\{y,z\})$,  whereas the formula $x = y$ does not admit variable 
decomposability with respect to $\Pi = (\{x\},\{y\})$. A special type of
variable decomposition that has played a crucial role in last decade is the
so-called \emph{monadic decomposition}, where the given $\Pi = \{X_i\}_{i=1}^n$
satisfies that $|X_i| = 1$, meaning that the given formula $\varphi$ can be
written as a boolean combination of monadic predicates.

\paragraph{History and Motivation.} The problem of variable decomposability was
first systematically studied by Libkin in the early 2000s \cite{libkin:2003},
who was primarily motivated by speeding up quantifier eliminations in
constraint database applications. Libkin developed a sufficient condition for 
inferring decidability of variable decomposability for various first-order 
theories (among others, the theory of real fields and the theory of automatic
structures). The problem of monadic decomposability was introduced and
systematically studied by Veanes et al.  \cite{veanes:2017}. They first noted 
that existing results on variable decomposability at that time concentrated 
mostly on first-order theories, whereby techniques do not immediately transfer 
to 
\emph{quantifier-free theories}, which play a more important role in SMT. The 
authors then set out to develop machineries for monadic decomposability for
generic SMT theories. This includes an efficient generic semi-algorithm, which 
is guaranteed to output a monadic decomposition in a compact representation of
``if-then-else'' formulas. Secondly, they authors provided algorithms for
checking nondecomposability for various major SMT theories (including EUF, 
i.e., the theory of equality with uninterpreted functions). The authors also
provided the first comprehensive account of the applications of
monadic decompositions (as well as variable decomposability), including 
compiler optimization, theorem proving, program analysis, and string analysis.

It is fair to say that other existing results regarding variable/monadic
decompositions essentially build on the aforementioned results
\cite{libkin:2003,veanes:2017}. For example, one could analyze the complexity
of checking decomposability, which could be run before attempting to generate a
variable/monadic decomposition (e.g. using the generic semi-algorithm of
\cite{veanes:2017}). This line of work was initiated in Libkin's paper
\cite{libkin:2003}, where he derived polynomial-time solvability of variable
decomposability
over quantifier-free formulas in the theory of real-closed fields with any fixed
number of variables; his algorithm runs in double-exponential time when the
number of variables is not fixed. Several further complexity results are
available over other theories. For example, Hague et al. \cite{hague:2020}
showed coNP-completeness for both variable/monadic decomposability over
qunatifier-free Linear Integer Arithmetic (LIA). Barcelo et al.
\cite{barcelo:2019} showed NL-completeness (resp. PSPACE-completeness) for
quantifier-free theory of automatic structures, when the formulas are
represented as a single deterministic (resp. nondeterministic) synchronous
automaton. Another possible line of work is to provide a new semi-algorithm for 
variable/monadic decompositions over specific theories, e.g., the recent work of
Markgraf et al. \cite{markgraf:2021}, which develops an exact learning
algorithm to speed up the generation of a monadic decomposition.

\paragraph{Contributions.} The main contribution of our paper is a precise
complexity of variable/monadic decomposability for LRA, i.e., we show that the
problem is coNP-complete. This substantially improved Libkin's double
exponential-time algorithm \cite{libkin:2003} for the problem. 
%Unlike the
%approach of \cite{libkin:20023} (which uses o-minimality and results in
%algebraic geometry), 
Geometrically the solution space of an LRA formula $\varphi(\bar x)$ can be
visualized as a finite union of the so-called \emph{e-convex polyhedra}. Here an
e-convex polyhedron \cite{rodriguez:2017}
is generated by linear systems contraining strict or
non-strict inequalities. The major difficulty in determining
variable/monadic decomposability of $\varphi$ lies in the presence of
\emph{union}. For example, 
\[
\varphi := x = y \wedge x \in [0,1] \wedge y \in [0,1]
\]
is not monadically decomposably, but $\varphi \vee (x \in [-1,1] \wedge y \in
[-1,1]$ \emph{is}. Therefore, we can\emph{not} simply analyze DNF-terms in 
$\varphi$ separately. Our main result is an algorithm that converts $\varphi$
into a ``normal form'' that allows us to then deduce monadic/variable
decomposability or non-decomposability. We furthermore show that this leads to a
polynomial witness for monadic/variable non-decomposability, i.e., a coNP
algorithm for decomposability. 
We have implemented a prototype of our algorithm. Based on our preliminary
experiments on various microbenchmarks, we report encouraging results.


==> toc.tex <==
% improve the styling of the table of contents (i.e., make section heading bold)

\makeatletter
\renewcommand*\l@section[2]
{%
	\ifnum \c@tocdepth >\z@
	\addpenalty \@secpenalty
	\addvspace {1.0em \@plus \p@ }%
	\setlength \@tempdima {1.5em}%
	\begingroup
	\parindent \z@
	\rightskip \@pnumwidth
	\parfillskip -\@pnumwidth
	\leavevmode \bfseries
	\advance \leftskip \@tempdima
	\hskip -\leftskip
	#1\nobreak % #1 is the section title
	\hfil
	\nobreak
	\hb@xt@ \@pnumwidth {\hss #2\kern -\p@ \kern \p@ } % #2 is the section page
	\par
	\endgroup
	\fi
}
\makeatother
